Stochastic Resource Allocation for Electricity Distribution Network Resilience

In recent years, it has become crucial to improve the resilience of electricity distribution networks (DNs) against storm-induced failures. Microgrids enabled by Distributed Energy Resources (DERs) can significantly help speed up re-energization of loads, particularly in the complete absence of bulk power supply. We describe an integrated approach which considers a pre-storm DER allocation problem under the uncertainty of failure scenarios as well as a post-storm dispatch problem in microgrids during the multi-period repair of the failed components. This problem is computationally challenging because the number of scenarios (resp. binary variables) increases exponentially (resp. quadratically) in the network size. Our overall solution approach for solving the resulting two-stage mixed-integer linear program (MILP) involves implementing the sample average approximation (SAA) method and Benders Decomposition. Additionally, we implement a greedy approach to reduce the computational time requirements of the post-storm repair scheduling and dispatch problem. The optimality of the resulting solution is evaluated on a modified IEEE 36-node network.

==> caseStudy.tex <==
\begin{figure}[htbp!]
%\vspace{-10mm}
	\centering
	\tikzset{every node/.append ={font size=tiny}} 
	%	\tikzstyle{mynode} = {circle, minimum size=0.5pt, inner sep = 2}
	%	\tikzstyle{dnnode}=mynode+fill=cyan]
	\tikzstyle{dnnode}=[draw,circle, minimum size=0.5pt, inner sep = 2]
	\tikzstyle{dnedge}=[-, line width=1pt]
	\tikzstyle{vuledge}=[-, line width=3pt, red!70]
	\tikzstyle{swind}=[->, line width=2pt, blue!25, >=latex']
	\tikzstyle{dernode}=[circle, fill=blue, minimum size=0.5pt, inner sep = 2]
	\tikzstyle{blackoutnode}=[circle, fill=black, minimum size=0.5pt, inner sep = 2]
	\tikzstyle{graynode}=[draw=black, pattern=north west lines, fill = black, circle,  minimum size=0.5pt, inner sep = 2, fill opacity=0.2]
	\tikzstyle{graynodes}=[circle, pattern=north west lines, fill = black, minimum size=0.5pt, inner sep = 2,fill opacity = 0.6]
	\tikzstyle{failededge}=[-, densely dotted]
	\def \drawgrid {\draw[step=1,gray, ultra thin, draw opacity = 0.5] (0,0) grid (3,4);}
	\def \drawSubstation {\draw[-, line width = 2pt] (0.8,4.05) -- (2.2,4.05)  node [midway,above] {};}
	\def \drawZero {\node[dnnode] (0) at (1.5,3.85) {};}
	\def \drawA {\node[dnnode] (A) at (1.5,3.0) {};}
	\def \drawAone {\node[dnnode] (A1) at (2,2.5) {};}
	\def \drawAtwo {		\node[dnnode] (A2) at (2.75,2.75) {};}
	\def \drawB {\node[dnnode] (B) at (0.25,2.75) {} ;}
	\def \drawC {\node[dnnode] (C) at (0.25,1.5) {} ;}
	\def \drawD {\node[dnnode] (D) at (1.5,1.25) {} ;}
	\def \drawDone {\node[dnnode] (D1) at (1.5,0.25) {} ;}
	\def \drawDtwo {\node[dnnode] (D2) at (0.5,0.25) {} ;}
	\def \drawDthree {\node[dnnode] (D3) at (1.5,2.00) {} ;}
	\def \drawE {\node[dnnode] (E) at (2.75,1.25) {} ;}
	\def \drawF {\node[dnnode] (F) at (2.75,0.50) {} ;}
	\subfloat[]{\label{subfig:nominal}
		\begin{tikzpicture}[scale=0.6,every node/.append ={font size=tiny}]
		
		\drawgrid \drawSubstation
		
		\drawZero \drawA \drawAone \drawAtwo \drawB \drawC \drawD \drawDone \drawDtwo \drawDthree \drawE \drawF 
		
		\foreach \from/\to in {0/A, A/B, A/A1, A1/A2, B/C, C/D, D/E, D/D1, D1/D2, D/D3, E/F}
		\draw[dnedge] (\from) -- (\to);		
		
		%		\node[label={ [label distance=0]-120:\footnotesize 0 }] at (0) {};
		\node at (0) {\tiny $\text{0}$};
		\node at (A) {\tiny $\text{A}$};
		\node at (A1) {\tiny $\text{G}$};
		\node at (A2) {\tiny $\text{H}$};
		\node at (B) {\tiny $\text{B}$};
		\node at (C) {\tiny $\text{C}$};
		\node at (D) {\tiny $\text{D}$};
		\node at (D1) {\tiny $\text{I}$};
		\node at (D2) {\tiny $\text{J}$};
		\node at (D3) {\tiny $\text{K}$};
		\node at (E) {\tiny $\text{E}$};
		\node at (F) {\tiny $\text{F}$};
		\end{tikzpicture}
	}
	\subfloat[]{\label{subfig:predictions}
		\begin{tikzpicture}[scale=0.6]
		\drawgrid \drawSubstation
		
		\drawZero \drawA \drawAone \drawAtwo \drawB \drawC \drawD \drawDone \drawDtwo \drawDthree \drawE \drawF 
		
		\node[dernode] (Dder) at (D) {} ;
		
		\foreach \from/\to in {0/A, A/B, A/A1, A1/A2, B/C, C/D, D/E, D/D1, D1/D2, D/D3, E/F}
		\draw[dnedge] (\from) -- (\to);		
		\foreach \from/\to in {0/A, B/C, D/E, D/D1, D/D3}
		\draw[vuledge] (\from) -- (\to);
		
		\foreach \mx/\my in {0.5/2.5, 2/3, 0.75/1.75, 2/2, 0.75/0.5, 2/0.75}	
		\draw[swind] (\mx,\my) to  (\mx+0.75,\my+0.25);
		\end{tikzpicture}
	}
	\subfloat[$\period = 0$]{\label{subfig:failures}
		\begin{tikzpicture}[scale=0.6]
		\drawgrid \drawSubstation
		
		\drawZero \drawA \drawAone \drawAtwo \drawB \drawC \drawD \drawDone \drawDtwo \drawDthree \drawE \drawF 
		
		\node[blackoutnode] (0) at (0) {};
		\node[blackoutnode] (A) at (A) {};
		\node[blackoutnode] (A1) at (A1) {};
		\node[blackoutnode] (A2) at (A2) {};
		\node[blackoutnode] (B) at (B) {} ;
		\node[dnnode] (C) at (C) {} ;
		\node[dnnode] (D) at (D) {} ;
		\node[blackoutnode] (D1) at (D1) {} ;
		\node[blackoutnode] (D2) at (D2) {} ;
		\node[blackoutnode] (D3) at (D3) {} ;
		\node[dernode] (Dder) at (D) {} ;
		\node[blackoutnode] (E) at (E) {} ;
		\node[blackoutnode] (F) at (F) {} ;
		
		\foreach \from/\to in { A/B, A/A1, A1/A2, C/D, D1/D2, E/F}
		\draw[dnedge] (\from) -- (\to);		
		\foreach \from/\to in {0/A, B/C, D/E, D/D1, D/D3}
		\draw[failededge] (\from) -- (\to);
		\end{tikzpicture}
	}
	\\	\subfloat[$\period = 1$]{\label{subfig:firstRepairs}
		\begin{tikzpicture}[scale=0.6]
		
		\drawgrid \drawSubstation
		
		\node[blackoutnode] (0) at (0) {};
		\node[blackoutnode] (A) at (A) {};
		\node[blackoutnode] (A1) at (A1) {};
		\node[blackoutnode] (A2) at (A2) {};
		\node[blackoutnode] (B) at (B) {} ;
		\node[graynode] (C) at (C) {} ;
		\node[dnnode] (D) at (D) {} ;
		\node[graynode] (D1) at (D1) {} ;
		\node[graynode] (D2) at (D2) {} ;
		\node[blackoutnode] (D3) at (D3) {} ;
		\node[dernode] (Dder) at (D) {} ;
		\node[graynode] (E) at (E) {} ;
		\node[graynode] (F) at (F) {} ;
		
		\foreach \from/\to in { A/B, A/A1, A1/A2, C/D, D/E, D/D1, D1/D2, E/F}
		\draw[dnedge] (\from) -- (\to);		
		\foreach \from/\to in {0/A,B/C, D/D3}
		\draw[failededge] (\from) -- (\to);
		
		\end{tikzpicture}
	}
	\subfloat[$\period = 2$]{\label{subfig:secondRepairs}
		\begin{tikzpicture}[scale=0.6]
		
		\drawgrid \drawSubstation
		\drawZero \drawA \drawAone \drawAtwo \drawB \drawC \drawD \drawDone \drawDtwo \drawDthree \drawE \drawF 
		
		\node[blackoutnode] (0b) at (0) {};
		\node[blackoutnode] (Ab) at (A) {};
		\node[blackoutnode] (A1b) at (A1) {};
		\node[blackoutnode] (A2b) at (A2) {};
		\node[graynodes] (Bb) at (B) {} ;
		\node[graynodes] (C) at (C) {} ;
		\node[dnnode] (D) at (D) {} ;
		\node[graynodes] (D1) at (D1) {} ;
		\node[graynodes] (D2) at (D2) {} ;
		\node[graynodes] (D3) at (D3) {} ;
		\node[dernode] (Dder) at (D) {} ;
		\node[graynodes] (E) at (E) {} ;
		\node[graynodes] (F) at (F) {} ;
		
		\foreach \from/\to in { A/B, A/A1, A1/A2, C/D, D/E, D/D1, D1/D2, E/F,B/C, D/D3}
		\draw[dnedge] (\from) -- (\to);		
		\foreach \from/\to in {0/A}
		\draw[failededge] (\from) -- (\to);
		
		\end{tikzpicture}
	}
	\subfloat[$\period = \nperiod$]{\label{subfig:reconnected}
		\begin{tikzpicture}[scale=0.6]
		\drawgrid \drawSubstation
		\drawZero \drawA \drawAone \drawAtwo \drawB \drawC \drawD \drawDone \drawDtwo \drawDthree \drawE \drawF 
		
		\foreach \from/\to in {0/A, A/B, A/A1, A1/A2, B/C, C/D, D/E, D/D1, D1/D2, D/D3, E/F}
		\draw[dnedge] (\from) -- (\to);		
		\foreach \from/\to in {0/A, B/C, D/E, D/D1, D/D3}
		\draw[dnedge] (\from) -- (\to);
		\end{tikzpicture}
	}
	\caption{The subfigures show (a) nominal DN (white nodes indicate no load control), (b) pre-storm DER allocation based on storm forecast (blue node denotes DER allocation, red lines illustrate a disruption scenario), (c) microgrid islands (dotted lines indicate failed lines, black nodes denote the unserved loads), (d) partial line repairs enable partial load restoration (light gray nodes), (e) line repairs completed leading to more load restoration, although with more load control than before (dark gray nodes), and (f) reconnection to main grid and restoration of nominal performance. }
	\label{fig:Schematic}
\end{figure}
